Impact of Decoding Methods on Human Alignment of Conversational LLMs

To be included into chatbot systems, Large language models (LLMs) must be aligned with human conversational conventions. However, being trained mainly on web-scraped data gives existing LLMs a voice closer to informational text than actual human speech. In this paper, we examine the effect of decoding methods on the alignment between LLM-generated and human conversations, including Beam Search, Top K Sampling, and Nucleus Sampling. We present new measures of alignment in substance, style, and psychometric orientation, and experiment with two conversation datasets. Our results provide subtle insights: better alignment is attributed to fewer beams in Beam Search and lower values of P in Nucleus Sampling. We also find that task-oriented and open-ended datasets perform differently in terms of alignment, indicating the significance of taking into account the context of the interaction.

==> avg_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!ht]
\small
\centering
\begin{tabular}{c|ccccc|c}
\toprule
\multicolumn{1}{l}{} & Politeness                   & Negotiation                  & Self Concept                 & Empathy                      & Verbosity                    & Semantic Similarity                   \\ \midrule
Base                 & 0.307                        & 0.107                        & 0.641                        & 0.657                        & 0.185                        & 0.525                                 \\ \midrule
\multicolumn{7}{c}{Number of Beams}                                                                                                                                                                                     \\ \midrule
2                    & {\color[HTML]{C00000} 0.308} & \textbf{0.097}               & 0.585                        & 0.648                        & 0.168                        & 0.498                                 \\
4                    & 0.306                        & 0.120                        & 0.584                        & \textbf{0.635}               & \textbf{0.165}               & \textbf{0.507}                        \\
6                    & 0.304                        & {\color[HTML]{C00000} 0.121} & {\color[HTML]{C00000} 0.606} & {\color[HTML]{C00000} 0.653} & 0.189                        & {\color[HTML]{C00000} 0.497} \\
8                    & \textbf{0.304}               & 0.109                        & \textbf{0.584}               & 0.651                        & {\color[HTML]{C00000} 0.190} & 0.499                                 \\ \midrule
\multicolumn{7}{c}{P Value}                                                                                                                                                                                             \\ \midrule
0                    & 0.314                        & 0.093                        & 0.593                        & \textbf{0.627}               & 0.195                        & 0.508                                 \\
0.5                  & {\color[HTML]{C00000} 0.317} & {\color[HTML]{C00000} 0.130} & 0.625                        & 0.631                        & \textbf{0.163}               & 0.500                                 \\
0.6                  & 0.314                        & 0.095                        & 0.604                        & 0.647                        & 0.189                        & 0.507                                 \\
0.7                  & 0.311                        & \textbf{0.088}               & \textbf{0.580}               & 0.647                        & 0.207                        & \textbf{0.519}                        \\
0.8                  & 0.315                        & 0.121                        & 0.634                        & 0.656                        & {\color[HTML]{C00000} 0.209} & {\color[HTML]{C00000} 0.491} \\
0.9                  & \textbf{0.307}               & 0.116                        & 0.614                        & {\color[HTML]{C00000} 0.667} & 0.199                        & 0.497                                 \\
1                    & 0.311                        & 0.120                        & {\color[HTML]{C00000} 0.637} & 0.653                        & 0.189                        & 0.514                                 \\ \midrule
\multicolumn{7}{c}{K Value}                                                                                                                                                                                             \\ \midrule
1                    & 0.314                        & 0.098                        & 0.593                        & \textbf{0.629}               & 0.196                        & 0.512                                 \\
20                   & 0.316                        & 0.118                        & 0.619                        & 0.657                        & 0.192                        & 0.492                                 \\
30                   & 0.316                        & {\color[HTML]{C00000} 0.126} & {\color[HTML]{C00000} 0.629} & 0.638                        & {\color[HTML]{C00000} 0.204} & 0.501                                 \\
40                   & {\color[HTML]{C00000} 0.317} & 0.097                        & \textbf{0.585}               & 0.659                        & 0.203                        & {\color[HTML]{C00000} 0.465} \\
50                   & 0.314                        & 0.108                        & 0.623                        & 0.649                        & \textbf{0.188}               & 0.488                                 \\
60                   & 0.313                        & 0.108                        & 0.602                        & 0.653                        & 0.191                        & 0.505                                 \\
70                   & \textbf{0.312}               & \textbf{0.084}               & 0.599                        & {\color[HTML]{C00000} 0.663} & 0.194                        & \textbf{0.514}                        \\ \bottomrule
\end{tabular}
\caption{Scores on the six psychological metrics averaged across all conversations in both datasets (BOLT, CraigslistBargains) and generated using both LLMs (Llama 3, Llama 3 Instruct). Higher values are better for Semantic Similarity and lower values are better for the other five measures. Scores marked with a * are statistically significant (p < 0.05).}
\label{avg_table}
\end{table*}

==> graph_figure.tex <==
% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{latex/graphs/bolt_sdt.png}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{latex/graphs/bolt_sdt.png}
%          \caption{$y=3\sin x$}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{latex/graphs/bolt_sdt.png}
%          \caption{$y=5/x$}
%          \label{fig:five over x}
%      \end{subfigure}
%         \caption{Three simple graphs}
%         \label{fig:three graphs}
% \end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{latex/graphs/bolt_polite.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{latex/graphs/bolt_harbingers.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_polite.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_harbingers.png}
    \end{subfigure}
    
    \medskip
    
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/bolt_sdt.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/bolt_empathy.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_sdt.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_empathy.png}
    \end{subfigure}
    
    \medskip
    
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/bolt_length.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/bolt_full-similarity.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_length.png}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\linewidth]{latex/graphs/craigslist_full-similarity.png}
    \end{subfigure}
    \caption{}
\end{figure*}

